SWAM: SDN-based Wi-Fi Small Cells with Joint Access-Backhaul and Multi-Tenant Capabilities

Dense deployments of Small Cells are required to deliver the capacity promised by 5G networks. In this paper we present SWAM, a system that builds on commodity Wi-Fi routers with multiple wireless interfaces to provide a wireless access infrastructure supporting multi-tenancy, mobility, and integrated wireless access and backhaul. An infrastructure provider can deploy inexpensive SWAM nodes to cover a given geographical area, and re-sell this capacity to provide on-demand connectivity for Mobile Network Operators. Our main contribution is the design of the SWAM datapath and control plane, which are inspired by the overlay techniques used to enable multi-tenancy in data-center networks. We prototype SWAM in an office wireless testbed, and validate experimentally its functionality.

==> acknowledgement.tex <==
\section{Acknowledgements}
This work has been supported by the European Commission under the 5G-PICTURE project (grant agreement 762057). Some authors of this work are also supported by the Spanish ministery under grant TEC2016-76795-C6-2-R.
